LSM: Learning Subspace Minimization for Low-level Vision

We study the energy minimization problem in low-level vision tasks from a novel perspective. We replace the heuristic regularization term with a learnable subspace constraint, and preserve the data term to exploit domain knowledge derived from the first principle of a task. This learning subspace minimization (LSM) framework unifies the network structures and the parameters for many low-level vision tasks, which allows us to train a single network for multiple tasks simultaneously with completely shared parameters, and even generalizes the trained network to an unseen task as long as its data term can be formulated. We demonstrate our LSM framework on four low-level tasks including interactive image segmentation, video segmentation, stereo matching, and optical flow, and validate the network on various datasets. The experiments show that the proposed LSM generates state-of-the-art results with smaller model size, faster training convergence, and real-time inference.

==> flow.tex <==

\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\subsection{Optical Flow}
The second task is optical flow, a two-dimensional dense correspondence estimation problem.
\paragraph{Problem Formulation}
Let $(u,v)$ be the 2D motion vector that warps the pixel coordinate $\vp$ to $\vw=(x+u,y+v)$ in the source image S. The feature channels should also be consistent and yield the pixel-wise objective function:
\begin{equation}
E(u,v)=\sum_{c=1}^{C}\|S_c(\vw)-T_c(\vp)\|_{2}^{2}.
\end{equation}
Simiar to disparity estimation, we also apply coarse-to-fine strategy and solve for an incremental update at each iteration by the feed-forward algorithm:
\begin{equation}
\begin{aligned}
\Delta u^{*},\Delta v^{*}&=\argmin\sum_{c=1}^{C}\|S_c(\vw+\begin{bmatrix}
           \Delta u\\
           \Delta v 
         \end{bmatrix})-T_c(\vp)\|_{2}^{2}\\
&\approx\argmin\sum_{c=1}^{C}\|S_c(\vw)+[\frac{\partial S_c}{\partial \vw_{x}},\frac{\partial S_c}{\partial \vw_{y}}]\begin{bmatrix}
           \Delta u\\
           \Delta v 
         \end{bmatrix}-T_c(\vp)\|_{2}^{2}\\
% &={\left[ {\begin{array}{cc}
%    \sum (\frac{\partial S_c}{\partial \vw_{x}})^{2}  &\sum(\frac{\partial S_c}{\partial \vw_{x}})(\frac{\partial S_c}{\partial \vw_{y}}) \\
%    \sum (\frac{\partial S_c}{\partial \vw_{x}})(\frac{\partial S_c}{\partial \vw_{y}}) & \sum{(\frac{\partial S_c}{\partial \vw_{y}})}^{2} \\
%   \end{array} } \right]}^{-1}
%   \left[ {\begin{array}{c}
%    \sum \frac{\partial S_c}{\partial \vw_{x}}[S_c(\vw)-T_c(\vp)]\\
%    \sum \frac{\partial S_c}{\partial \vw_{y}}[S_c(\vw)-T_c(\vp)]\\
%   \end{array}} \right]\\
&={\left[ {\begin{array}{cc}
   \sum g_{x}^{2}  & \sum g_{x}g_{y} \\
   \sum g_{x}g_{y} & \sum g_{y}^{2}  \\
  \end{array} } \right]}^{-1}
  \left[ {\begin{array}{c}
   \sum s_{x}\\
   \sum s_{y}\\
  \end{array}} \right],
\end{aligned}
\label{equ:flow0}
\end{equation}
where $g_{x}$ and $g_{y}$ represent the spatial gradient of feature maps along x-axis and y-axis respectively, and $s_{x}$ and $s_{y}$ is the steepest descent update along x-axis and y-axis. 
Then the dense flow field update $\Delta \vf$ can be solved by an unconstrained quadratic minimization:
\begin{equation}
\Delta\vf^{*}=\argmin\frac{1}{2}\Delta \vf^{\top}\left[ {\begin{array}{cc}
   \mH_{xx}  & \mH_{xy} \\
   \mH_{xy} &  \mH_{yy}  \\
  \end{array} } \right]\Delta\vf-[\vs_x^{\top},\vs_y^{\top}]\Delta \vf,
\label{equ:flow1}
\end{equation}
where $\mH_{xx}=diag(G_{xx})$, $\mH_{yy}=diag(G_{yy})$, $\mH_{xy}=diag(G_{xy})$ are the corresponding diagonal matrix containing the gradient quantities for all pixels.\\
Solving~\equref{flow1} is also equivalent to operating~\equref{flow0} at all pixels. Following the formulation in~\equref{lsm_d}, we constraint the horizontal and vertical components of the dense flow field update $\Delta\vf=[u_{1},u_{2}\cdots u_{N},v_{1},v_{2}\cdots v_{N}]^{\top}$ onto two independent subspaces and solve for the linear combination coefficients $\vc_{u}$ and $\vc_{v}$:
% \scalebox{0.95}{
\begin{equation}
\begin{aligned}
\vc_{u}^{*},\vc_{v}^{*}=\argmin\frac{1}{2}\left[\begin{array}{c}\vc_{u}\\\vc_{v}\end{array}\right]^{\top}\left[ {\begin{array}{cc}
   \mV_{u}^{\top}\mH_{xx}\mV_{u} & \mV_{u}^{\top}\mH_{xy}\mV_{v} \\
   \mV_{v}^{\top}\mH_{xy}\mV_{u} &  \mV_{v}^{\top}\mH_{yy}\mV_{v} \\
  \end{array} } \right]\left[\begin{array}{c}\vc_{u}\\\vc_{v}\end{array}\right]-[\vs_x^{\top}\mV_{u},\vs_y^{\top}\mV_{v}]\left[\begin{array}{c}\vc_{u}\\\vc_{v}\end{array}\right].
\end{aligned}
\label{equ:flow2}
\end{equation}
% }
\paragraph{Learning Subspace} We apply the same principles and reuse the same network structures as in disparity estimation. However, concatenating the quantites in~\equref{flow0} generates minimization context features with different number of channels. In order to unify the subspace prediction for both disparity estimation and optical flow, we transform~\equref{flow0} by Cramer's rule~\citep{Higham}:
\begin{equation}
\begin{aligned}
\Delta u^{*}&=det\left|{\begin{array}{cc}
   \sum s_{x}  & \sum g_{x}g_{y} \\
   \sum s_{y}  & \sum g_{y}^{2}  \\
  \end{array} } \right|\bigg/det\left|{\begin{array}{cc}
   \sum g_{x}^{2}  & \sum g_{x}g_{y} \\
   \sum g_{x}g_{y} & \sum g_{y}^{2}  \\
  \end{array} } \right|\\
\Delta v^{*}&=det\left|{\begin{array}{cc}
   \sum g_{x}g_{y} &\sum s_{x}\\
   \sum g_{y}^{2}  &\sum s_{y}\\
  \end{array} } \right|\bigg/det\left|{\begin{array}{cc}
   \sum g_{x}^{2}  & \sum g_{x}g_{y} \\
   \sum g_{x}g_{y} & \sum g_{y}^{2}  \\
  \end{array} } \right|,
\end{aligned}
\label{equ:flow3}
\end{equation}
where $det|\bigcdot|$ denotes the determinant value of a matrix.~\equref{flow3} enables sharing network structures between disparity estimation and optical flow because averaging the determinant values in~\equref{flow3} every $G$ channels generates $M$ channel minimization context features for the horizontal and the vertical components $\Delta \vf$ respectively, which is identical to the disparity estimation. In addition,~\equref{flow3} even enables sharing network parameters because the determinant value gives the scaling factor and the orientation induced by a matrix, which has similar interpretations as the steepest descent update and the gradient norm. Please refer to the~\emph{supplementary materials} for detailed proof.


==> relation2reg.tex <==
\paragraph{Relation to Regularization Term}
\ping{I don't understand Equation 5, so I don't understand this paragraph. It also appears unnecessary and might be moved to supplementary.}\chengzhou{the reason I put it is because 1. Eq.5 maintain the subspace constraint 2. Eq.5 is better as validated in the ablation study 3. it estabilish the relation to regularziaton term and then we can disscuss the adavantages over regularization term based on the matrix $\mR$.}
The~\equref{min_proj} not only maintains the subspace constraint but also establishes the relation to~\equref{1} that contains the regularization term and is solved iteratively as:
\begin{equation}
\min_{\Delta\vx}\frac{1}{2}\Delta \vx^{\top}(\mD+\mR)\Delta\vx+(\vd+\mR\vx)^{\top}\Delta \vx,
\label{equ:iter}
\end{equation}
where $\mR$ contains the second-order derivatives of the regularization term $R(\vx)$ and is termed as the generalized laplacian filtering matrix, $\mR\vx$ is the first order derivative vector.

\begin{prop}\label{prop} 
If $\mR=\mD(\mP-\mI)$, and $\Delta \vx$ is a solution to \equref{iter}, its lower dimensional representation (coefficients)~$\vc=(\mV^{\top}\mV)^{-1}\mV^{\top}\Delta \vx$ will be the solution to~\equref{min_proj}.
\end{prop}

\begin{proof}
Let $\mR=\mD(\mP-\mI)$, so\chengzhou{move proof to supplementary?} 
%and $\Delta x$ is a solution to~\equref{iter} that satisfies the second-order optimality condition $(\mD+\mR)\Delta \vx+(\vd+\vl)=\boldsymbol{0}$, therefore:
\begin{align*}
(\mD+\mR)\Delta \vx&=\\
&=[\mD+\mD(\mP-\mI)]\Delta \vx\\
&=(\mD+\mD\mP-\mD)\Delta \vx\\
&=(\mD\mP)\Delta \vx\\
&=\mD\mV(\mV^{\top}\mV)^{-1}\mV^{\top}\Delta \vx\\
&=\mD\mV[(\mV^{\top}\mV)^{-1}\mV^{\top}\Delta \vx]\\
&=\mD\mV\vc.
\end{align*} 
Since $\Delta \vx$ is a solution to~\equref{iter} which satisfies the second-order optimality condition $(\mD+\mR)\Delta \vx=-(\vd+\mR\vx)$,
\begin{align*}
\mV^{\top}\mD\mV\vc&=\\
&=-\mV^{\top}(\vd+\mR\vx)\\
&=-\mV^{\top}[\vd+\mD(\mP-\mI)\vx]\\
&=-\mV^{\top}(\vd+\mD\vr),
\end{align*} 
which is the second-order optimality condition for~\equref{min_proj}, and $\vc=-(\mV^{\top}\mD\mV)^{-1}\mV^{\top}(\vd+\mD\vr)$.\qedhere
\end{proof} 
The Proposition.\ref{prop} shows the relation between the proposed LSM framework and conventional variational minimization with regularization term. But it does not mean that they are identical to each other.

In~\equref{iter}, $\mR$ is manually defined according to the regularization term. If $R(\vx)$ is the Tikhonov regularization ($L2$ smoothness term), multiplication with $\mR$ can be implemented efficiently as laplacian filtering, but its performance is poor. More sophisticated solution gives better performance, but is complicated and expensive, e.g. $\mR$ is dense for non-local regularization~\citep{NONLOCALS,TV,nonlocal2,nonlocalsup} and can be approximated using high-dimensional filtering~\citep{DomainTransform,Lattice}, but the approximated multiplication still costs more than one minute~\citep{NONLOCALS}. 

In contrast, our LSM framework learns to predict the subspace $\mathcal{V}$ from data, so $\mR=\mD(\mP-\mI)$ adapts to each sample and does not have a fixed form. Since we incorporate the minimization context in subspace prediction, $\mR$ progressively evolves and guides the minimization instead of conventionally being defined only on the image context and fixed for all iterations. The LSM framework is also efficient, e.g. we can compute $\mV^{\top}\mR\vx$ as $(\mV^{\top}\mD\mV)(\mV^{\top}\mV)^{-1}\mV^{\top}\vx-\mV^{\top}\mD\vx$, which avoids constructing the dense $N\text{-by-}N$ matrix $\mR$ and the intractable multiplication with it.\chengzhou{The advantage of easy end-to-end training is introduced in the overview, move here?} 
